Towards a Practical, Budget-Oblivious Algorithm for the Adwords Problem under Small Bids

Motivated by recent insights into the online bipartite matching problem (\textsc{OBM}), our goal was to extend the optimal algorithm for it, namely \textsc{Ranking}, all the way to the special case of adwords problem, called \textsc{Small}, in which bids are small compared to budgets; the latter has been of considerable practical significance in ad auctions \cite{MSVV}. The attractive feature of our approach was that it would yield a {\em budget-oblivious algorithm}, i.e., the algorithm would not need to know budgets of advertisers and therefore could be used in autobidding platforms. We were successful in obtaining an optimal, budget-oblivious algorithm for \textsc{Single-Valued}, under which each advertiser can make bids of one value only. However, our next extension, to \textsc{Small}, failed because of a fundamental reason, namely failure of the {\em No-Surpassing Property}. Since the probabilistic ideas underlying our algorithm are quite substantial, we have stated them formally, after assuming the No-Surpassing Property, and we leave the open problem of removing this assumption. With the help of two undergrads, we conducted extensive experiments on our algorithm on randomly generated instances. Our findings are that the No-Surpassing Property fails less than $2\%$ of the time and that the performance of our algorithms for \textsc{Single-Valued} and \textsc{Small} are comparable to that of \cite{MSVV}. If further experiments confirm this, our algorithm may be useful as such in practice, especially because of its budget-obliviousness.

==> Online.tex <==

\section{Online Bipartite Matching: \textsc{Ranking}}
\label{sec.bipartite}
 
 
Algorithm \ref{alg.Ranking} presents an optimal algorithm for \textsc{OBM}. Note that this algorithm picks a random permutation of goods only once. Its competitive ratio is $(1 - {\frac 1 e})$, as shown in Theorem \ref{thm.ranking}. Furthermore, as shown in \cite{KVV}, it is an optimal online bipartite matching algorithm: no randomized algorithm can do better, up to an $o(1)$ term.  

We will analyze Algorithm \ref{alg.Ranking2} which is equivalent to Algorithm \ref{alg.Ranking} and  operates as follows. Before the execution of Step (1), the adversary determines the order in which buyers will arrive, say $\cO(B)$. In Step (1), each good $j$ is assigned a {\em price} $p_j = e^{w_j - 1}$, where $w_j$, called the {\em rank} of $j$, is picked at random from $[0, 1]$; observe that $p_j \in [{1 \over e}, 1]$. In Step (2), buyers will arrive in the order $\cO(B)$, picked by the adversary, and will be matched to the cheapest available good. With probability 1 all $n$ prices are distinct and sorting the goods by increasing prices results in a random permutation. Furthermore, since Algorithm \ref{alg.Ranking2} uses this sorted order only and is oblivious of the actual prices, it is equivalent to Algorithm \ref{alg.Ranking}. As we will see, the random variables representing actual prices are crucially important as well -- in the analysis. We remark that for the generalizations of \textsc{OBM} studied in this paper, the prices are used not only in the analysis, but also by the algorithms.    


\begin{figure}

	\begin{wbox}
		\begin{alg}
		\label{alg.Ranking}
		{\bf (Algorithm \textsc{Ranking})}\\
		\\
		\begin{enumerate}
			\item {\bf Initialization:} Pick a random permutation, $\pi$, of the goods in $S$. 			
		\bigskip
			\item {\bf Online buyer arrival:} When a buyer, say $i$, arrives, match her to the first unmatched good she likes in the order $\pi$; if none, leave $i$ unmatched.
		\end{enumerate} 
		\bigskip
		Output the matching, $M$, found.
		\end{alg}
	\end{wbox}
\end{figure} 


\bigskip


\subsection{Analysis of \textsc{Ranking}}
\label{sec.analysis}

We will use an {\em economic setting} for analyzing Algorithm \ref{alg.Ranking2} as follows. Each buyer $i$ has {\em unit-demand} and {\em 0/1 valuations} over the goods she likes, i.e., she accrues unit utility from each good she likes, and she wishes to get at most one of them. The latter set is precisely the set of neighbors of $i$ in $G$. If on arrival of $i$ there are several of these which are still unmatched, $i$ will pick one having the smallest price \footnote{As stated above, with probability 1 there are no ties.}. Therefore the buyers will maximize their utility as defined below.

	For analyzing this algorithm, we will define two sets of random variables, $u_i$ for $i \in B$ and $r_j$, for $j \in S$. These will be called utility of buyer $i$ and revenue of good $j$, respectively. Each run of \textsc{Ranking} defines these random variables as follows. If \textsc{Ranking} matches buyer $i$ to good $j$, then define $u_i = 1 - p_j$ and $r_j = p_j$, where $p_j$ is the price of good $j$ in this run of \textsc{Ranking}. Clearly, $p_j$ is also a random variable, which is defined by Step (1) of the algorithm. If $i$ remains unmatched, define $u_i = 0$, and if $j$ remains unmatched, define $r_j = 0$. Observe that for each good $j$, $p_j \in [{1 \over e}, 1]$ and for each buyer $i$, $u_i \in [0, 1 - {1 \over e}]$. Let $M$ be the matching produced by \textsc{Ranking} and let random variable $|M|$ denote its size. 

Lemma \ref{lem.add} pulls apart the contribution of each matched edge $(i, j)$ into $u_i$ and $r_j$. Next, we established in Lemma \ref{lem.edge} that for each edge $(i, j)$ in the graph, the total expected contribution of $u_i$ and $r_j$ is at least $1 - {1 \over e}$. Then, linearity of expectation allows us to reassemble the $2n$ terms in the right hand side of Lemma \ref{lem.add} so they are aligned with a perfect matching in $G$, and this yields Theorem \ref{thm.ranking}.

\bigskip

\begin{lemma}
	\label{lem.add}
	\[ \bE [|M|] \ =  \sum_i^n {\bE \left[ {u_i} \right]} \ + \   \sum_j^n {\bE[r_j]}  .\]
\end{lemma}

\begin{proof}
	By definition of the random variables, 
		\[ \bE [|M|] \ = \bE \left[ \sum_{i = 1}^n {u_i} \ + \ \sum_{j = 1}^n {r_j} \right] 
		\ =  \sum_i^n {\bE \left[ {u_i} \right]} \ + \   \sum_j^n {\bE[r_j]}   ,\]
where the first equality follows from the fact that if $(i, j) \in M$ then $u_i + r_j = 1$ and the second follows from linearity of expectation.  
\end{proof}

\bigskip


\setcounter{figure}{1} 
%\begin{figure}[H]

\begin{figure}

	\begin{wbox}
		\begin{alg}
		\label{alg.Ranking2}
		{\bf (Algorithm \textsc{Ranking}: Economic Viewpoint)}\\
		\\
	
		\begin{enumerate}
			\item {\bf Initialization:} $\forall j \in S$: \ \ Pick $w_j$ independently and uniformly from $[0, 1]$. \\
			Set price \ $p_j \leftarrow e^{w_j - 1}$.
			
		\bigskip
			\item {\bf Online buyer arrival:} When a buyer, say $i$, arrives, match her to the cheapest unmatched good she likes; if none, leave $i$ unmatched.
		\end{enumerate} 
		\bigskip
		Output the matching, $M$, found.
		\end{alg}
	\end{wbox}
\end{figure} 




While running Algorithm \ref{alg.Ranking2}, assume that the adversary has picked the order of arrival of buyers, say $\cO(B)$, and Step (1) has been executed. We next define several ways of executing Step (2). Let $\cR$ denote the run of Step (2) on the entire graph $G$.  Corresponding to each good $j$, let $G_j$ denote graph $G$ with vertex $j$ removed. Define $\cR_j$ to be the run of Step (2) on graph $G_j$. 

	
\bigskip

Lemma \ref{lem.subset-j} and Corollary \ref{cor.subset-j} establish a relationship between the sets of available goods for a buyer $i$ in the two runs $\cR$ and $\cR_j$; the latter is crucially used in the proof of Lemma \ref{lem.R}. For ease of notation in proving these two facts, let us renumber the buyers so their order of arrival under $\cO(B)$ is $1, 2, \ldots n$. Let $T(i)$ and $T_j(i)$ denote the sets of unmatched goods at the time of arrival of buyer $i$ (i.e., just before the buyer $i$ gets matched) in the graphs $G$ and $G_j$, in runs $\cR$ and $\cR_j$, respectively. Similarly, let $S(i)$ and $S_j(i)$ denote the set of unmatched goods that buyer $i$ is incident to in $G$ and $G_j$, in runs $\cR$ and $\cR_j$, respectively.

We have assumed that Step (1) of Algorithm \ref{alg.Ranking2} has already been executed and a price $p_k$ has been assigned to each good $k$. With probability 1, the prices are all distinct. Let $F_1$ and $F_2$ be subsets of $S$ containing goods $k$ such that $p_k < p_j$ and $p_k > p_j$, respectively. 

\bigskip

\begin{lemma}
	\label{lem.subset-j}
	For each $i$, $1 \leq i \leq n$, the following hold:
	\begin{enumerate}
		\item $(T_j(i) \cap F_1) =  (T(i) \cap F_1)$.
		\item $(T_j(i) \cap F_2) \subseteq  (T(i) \cap F_2)$.
	\end{enumerate}
\end{lemma}

\begin{proof}
	Clearly, in both runs, $\cR$ and $\cR_j$, any buyer having an available good in $F_1$ will match to the most profitable one of these, without even considering the rest of the goods. Since $j \notin F_1$, the two runs behave in an identical manner on the set $F_1$, thereby proving the first statement. 
	 
	The proof of the second statement is by induction on $i$. The base case is trivially true since  $j \notin F_2$. Assume that the statement is true for $i = k$ and let us prove it for $i = k+1$. By the first statement, we need to consider only the case that there are no available goods for the $k^{th}$ buyer in $F_1$ in the runs $\cR$ and $\cR_j$. Assume that in run $\cR_j$, this buyer gets matched to good $l$; if she remains unmatched, we will take $l$ to be null. Clearly, $l$ is the most profitable good she is incident to in $T_j(k)$. Therefore, the most profitable good she is incident to in run $\cR$ is the best of $l$, the most profitable good in $T(k) - T_j(k)$, and $j$, in case it is available. In each of these cases, the induction step holds.
\end{proof}

In the corollary below, the first two statements follow from Lemma \ref{lem.subset-j} and the third statement follows from the first two. 

\bigskip

\begin{corollary}
	\label{cor.subset-j}
		For each $i$, $1 \leq i \leq n$, the following hold:
	\begin{enumerate}
		\item $(S_j(i) \cap F_1) =  (S(i) \cap F_1)$.
		\item $(S_j(i) \cap F_2) \subseteq  (S(i) \cap F_2)$.
		\item $S_j(i) \subseteq S(i)$.
	\end{enumerate}
\end{corollary}


\bigskip

Next we define a new random variable, $u_e$, for each edge $e = (i, j) \in E$. This is called the {\em threshold} for edge $e$ and is given in Definition \ref{def.threshold-Online}. It is critically used in the proofs of Lemmas \ref{lem.R} and \ref{lem.edge}.  

\bigskip

\begin{definition}
	\label{def.threshold-Online}
	Let $e = (i, j) \in E$ be an arbitrary edge in $G$. Define random variable, $u_e$, called the {\em threshold} for edge $e$, to be the utility of buyer $i$ in run $\cR_j$. Clearly, $u_e \in [0, 1 - {1 \over e}]$.
	\end{definition}
	
	\bigskip
	
\begin{property}
	\label{prop.OBM-no-surpass}
	{\bf (No-Surpassing for} \textsc{OBM})
	Let $p_j$ be such that the bid of $j$, namely $1 - p_j$, is better than the best bid that buyer $i$ gets in run $\cR_j$. Then, in run $\cR$, no bid to $i$ will surpass $1 - p_j$. 
\end{property}

\bigskip

\begin{lemma}
	\label{lem.OBM-no-surpassing}
	The No-Surpassing Property holds for \textsc{OBM}.
\end{lemma}

\begin{proof}
Suppose the bid of $j$, namely $1 - p_j$, is better than the best bid that buyer $i$ gets in run $\cR_j$. If so, $i$ gets no bid from $F_1$ in $\cR_j$; observe that they are all higher than $1 - p_j$. Now, by the first part of Corollary \ref{cor.subset-j}, $i$ gets no bid from $F_1$ in run $\cR$ as well, i.e., in run $\cR$, no bid to $i$ will surpass $1 - p_j$. 
\end{proof}

\bigskip

\begin{lemma}
	\label{lem.R}
	Corresponding to each edge $(i, j) \in E$, the following hold. 
	\begin{enumerate}
	    \item $u_i \geq u_e$, where $u_i$ and $u_e$ are the utilities of buyer $i$ in runs $\cR$ and $\cR_j$, respectively.
		\item  Let $z \in [0, 1 - {1 \over e}]$. Conditioned on $u_e = z$, if \ $p_j < 1 - z$, then $j$ will definitely be matched in run $\cR$. 
	\end{enumerate}
\end{lemma}

\begin{proof}
	{\bf 1).} By the third statement of Corollary \ref{cor.subset-j}, $i$ has more options in run $\cR$ as compared to run $\cR_j$, and therefore $u_i \geq u_e$.
	
			
	{\bf 2).} In run $\cR$, if $j$ is already matched when $i$ arrives, there is nothing to prove. Next assume that $j$ is not matched when $i$ arrives. The crux of the matter is that by Lemma \ref{lem.OBM-no-surpassing}, the No-Surpassing Property holds. Therefore, in run $\cR$, $i$ will not have any option that is better than $j$ and will therefore get matched to $j$. Since $1 - p_j > z$, $S_j(i) \cap F_1 = \emptyset$. Therefore by the first statement of Corollary \ref{cor.subset-j}, $S(i) \cap F_1 = \emptyset$. Since $i$ will get no bid better than $j$ in $\cR$, the no-surpassing property indeed holds and $i$ must get matched to $j$.
\end{proof}

\begin{remark}
	\label{rem.threshold-name}
	The random variable $u_e$ is called {\em threshold} because of the second statement of Lemma \ref{lem.R}. It defines a value such that whenever $p_j$ is smaller than this value, $j$ is definitely matched in run $\cR$.
\end{remark}

The intuitive reason for the next, and most crucial, lemma is the following. The smaller $u_e$ is, the larger is the range of values for $p_j$, namely $[0, 1 - u_e)$, over which $(i, j)$ will be matched and $j$ will accrue revenue of $p_j$. Integrating $p_j$ over this range, and adding $\bE [u_i]$ to it, gives the desired bound. Crucial to this argument is the fact that $p_j$ is independent of $u_e$. This follows from the fact that $u_e$ is determined by run $\cR_j$ on graph $G_j$, which does not contain vertex $j$. 


\bigskip

\begin{lemma}
	\label{lem.edge}
		Corresponding to each edge $(i, j) \in E$, 
	\[ \bE [u_i + r_j] \geq 1 - {\frac 1 e} . \]
\end{lemma}

\begin{proof}

	By the first part of Lemma \ref{lem.R}, $\bE [u_i] \geq \bE [u_e]$. 
	
	Next, we will lower bound $\bE [r_j]$. Let $z \in [0, 1 - {1 \over e}]$ and let us condition on the event $u_e = z$. The critical observation is that $u_e$ is determined by the run $\cR_j$. This  is conducted on graph $G_j$, which does not contain vertex $j$. Therefore $u_e$ is independent of $p_j$. 
	
	By the second part of Lemma \ref{lem.R}, $r_j = p_j$ whenever $p_j < 1 - z$. We will ignore the contribution to $\bE [r_j]$ when $p_j \geq 1 - z$. Let $w$ be s.t. $e^{w-1} = 1-z$.
	
	Now $p_j$ is obtained by picking $x$ uniformly at random from the interval $[0, 1]$ and outputting $e^{x-1}$. In particular, when $x \in [0, w)$, $p_j < 1-z$. If so, by the second part of Lemma \ref{lem.R}, $j$ is matched and revenue is accrued in $r_j$, see Figure \ref{fig.Revenue}. Therefore,  
		\[ \bE [r_j ~|~ u_e = z] \geq \int_0^{w} {e^{x-1} \ dx} \ = \ e^{w-1} - {\frac 1 e} \ = \ 1 - {\frac 1 e} - z .\]
		
		Let $f_{u_e}(z)$ be the probability density function of $u_e$; clearly, $f_{u_e}(z) = 0$ for $z \notin [0, 1 - {1 \over e}]$. 
		Therefore, 
			\[ \bE [r_j] \ = \ \bE [\bE [r_j ~|~ u_e] ] \ = \ \int_{z=0}^{1 - 1/e} {\bE [r_j ~|~ u_e = z] \cdot f_{u_e}(z) dz} \]
			\[ \geq \ 
	\int_{z=0}^{1 - 1/e} {\left(1 - {\frac 1 e} - z \right) \cdot f_{u_e}(z) dz} \ \ = \ \ 1 - {\frac 1 e} - \bE[u_e] ,\]
where the first equality follows from the law of total expectation and the inequality follows from  fact that we have ignored the contribution to $\bE [r_j ~|~ u_e]$ when $p_j \geq 1-z$. Hence we get
	\[ \bE [u_i + r_j] = \bE [u_i] + \bE [r_j] \geq 1 - {\frac 1 e} . \]
\end{proof}


\begin{figure}
	\centering
	\includegraphics[width=1.0\linewidth]{Revenue.pdf}
	\caption{The shaded area is a lower bound on $\bE [r_j ~|~ u_e = z]$.}
	\label{fig.Revenue}
\end{figure}



\begin{remark}
	Observe that Lemma \ref{lem.edge} is not a statement about $i$ and $j$ getting matched to each other, but about the utility accrued by $i$ and the revenue accrued by $j$ by being matched to various goods and buyers, respectively, over the randomization executed in Step (1) of Algorithm \ref{alg.Ranking2}.
	\end{remark}	
	
\bigskip

\begin{theorem}
	\label{thm.ranking}
	The competitive ratio of \textsc{Ranking} is at least $1 - {\frac 1 e}$.
\end{theorem}

\begin{proof}
	Let $P$ denote a perfect matching in $G$. The expected size of matching produced by \textsc{Ranking} is 
	\[ \bE \left[ |M| \right] \ = \ \sum_i^n {\bE \left[ {u_i} \right]} \ + \   \sum_j^n {\bE[r_j]}   	\ = \ \sum_{(i, j) \in P} {\bE [u_i + r_j]} \ \geq \ n \left( 1 - {\frac 1 e} \right) ,\]
	where the first equality uses Lemma \ref{lem.add}, the second follows from linearity of expectation and the inequality follows from Lemma \ref{lem.edge} and the fact that $|P| = n$. The theorem follows. 
\end{proof}

\begin{remark}
	\label{rem.not-perfect}
	In case $G$ does not have a perfect matching, let $P$ denote a maximum matching in $G$, of size $k$, say. Then summing ${\bE \left[ {u_i} \right]}$ and ${\bE[r_j]}$ over the the vertices $i$ and $j$ matched by $P$, we get that the expected size of matching produced by \textsc{Ranking} is at least $k \left( 1 - {\frac 1 e} \right)$.
\end{remark}


\begin{comment}
	\begin{lemma}
	\label{lem.S-subset-j}
	For each $i$, $1 \leq i \leq n$, the following hold:
	\begin{enumerate}
		\item $T_j(i) \subseteq T(i)$.
		\item $|T(i) - T_j(i)| \leq 1.$
	\end{enumerate}
\end{lemma}

\begin{proof}
	The proof is by induction on $i$. The base case is straightforward since $G$ and $G_j$ differ in only one good, namely $j$. Assume the statement is true for $i = k$ and let us prove it for $i = k+1$. If $T(k) = T_j(k)$, then the $(k+1)^{st}$ buyer behaves the same way in both runs and therefore $T(k+1) = T_j(k+1)$. 
	
	The main case is that $T(k) = T_j(k) \cup \{l\}$, for some good $l$. If $l \notin S(k)$, then clearly $T(k+1) = T_j(k+1) \cup \{l\}$. Next, assume $l \in S(k)$. Suppose $k$ is matched under $\cR_j$, say to good $l'$. Clearly, under $\cR$, $k$ will be matched to the cheaper of $l'$ and $l$. If former, then $T(k+1) = T_j(k+1) \cup \{l\}$, and if latter, then $T(k+1) = T_j(k+1) \cup \{l'\}$. Finally, suppose that $k$ is not matched under $\cR_j$. If so, $S(k) = \{l\}$ and $k$ will be matched to $l$ under $\cR$, therefore giving $T(k+1) = T_j(k+1)$.
\end{proof}

\begin{corollary}
	\label{cor.S-subset-j}
		For each $i$, $1 \leq i \leq n$, the following hold:
	\begin{enumerate}
		\item $S_j(i) \subseteq S(i)$.
		\item $|S(i) - S_j(i)| \leq 1$.
	\end{enumerate}
\end{corollary}
\end{comment}



